Search for a bound di-neutron by comparing $^3$He(e,e'p)d and $^3$H(e,e'p)X measurements

We report on a search for a bound di-neutron by comparing electron-induced proton-knockout $(e,e'p)$ measurements from Helium-3 ($^3$He) and Tritium ($^3$H). The measurements were performed at Jefferson Lab Hall A with a 4.326 GeV electron beam, and kinematics of large momentum transfer $Q^2 \approx 1.9$ (GeV/$c$)$^2$ and $x_B>1$, to minimize contributions from non quasi-elastic (QE) reaction mechanisms. Analyzing the measured $^3$He missing mass ($M_{miss}$) and missing energy ($E_{miss}$) distributions, we can distinguish the two-body break-up reaction, in which the residual proton-neutron system remains bound as a deuteron. In the $^3$H mirror case, under the exact same kinematic conditions, we do not identify a signature for a bound di-neutron with similar binding energy to that of the deuteron. We calculate exclusion limits as a function of the di-neutron binding energy and find that, for binding equivalent to the deuteron, the two-body break-up cross section on $^3$H is less than 0.9% of that on $^3$He in the measured kinematics at the 95% confidence level.

==> author.tex <==



\author{D.~Abrams} \affiliation{University of Virginia, Charlottesville, VA}
\author{H.~Albataineh} \affiliation{Texas A \& M University, Kingsville, TX}
\author{S.~Alsalmi } \affiliation{King Saud University, Riyadh, Kingdom of Saudi  Arabia}
\author{D.~Androic} \affiliation{University of Zagreb, Zagreb, Croatia}
\author{K.~Aniol} \affiliation{California State University , Los Angeles, CA}
\author{W.~Armstrong} \affiliation{Physics Division, Argonne National Laboratory, Lemont, IL}
\author{J.~Arrington} \affiliation{Physics Division, Argonne National Laboratory, Lemont, IL}
\author{H.~Atac} \affiliation{Temple University, Philadelphia, PA}
\author{T.~Averett} \affiliation{The College of William and Mary, Williamsburg, VA}
\author{C.~Ayerbe~Gayoso} \affiliation{The College of William and Mary, Williamsburg, VA}
%B                                                                                                                                                            
\author{X.~Bai} \affiliation{University of Virginia, Charlottesville, VA}
\author{J.~Bane} \affiliation{University of Tennessee, Knoxville, TN}
\author{S.~Barcus} \affiliation{The College of William and Mary, Williamsburg, VA}
\author{A.~Beck} \affiliation{Massachusetts Institute of Technology, Cambridge, MA}
\author{V.~Bellini} \affiliation{INFN Sezione di Catania, Italy}
\author{F. Benmokhtar} \affiliation{Duquesne University, Pittsburgh, PA}
\author{H.~Bhatt} \affiliation{Mississippi State University, Miss. State, MS}
\author{D.~Bhetuwal} \affiliation{Mississippi State University, Miss. State, MS}
\author{D.~Biswas} \affiliation{Hampton University , Hampton, VA}
\author{D.~Blyth} \affiliation{Physics Division, Argonne National Laboratory, Lemont, IL}
\author{W.~Boeglin} \affiliation{Florida International University, Miami, FL}
\author{D.~Bulumulla} \affiliation{Old Dominion University, Norfolk, VA}

%C                                                                                                                                                            
\author{A.~Camsonne} \affiliation{Jefferson Lab, Newport News, VA}
\author{J.~Castellanos} \affiliation{Florida International University, Miami, FL}
\author{J-P.~Chen} \affiliation{Jefferson Lab, Newport News, VA}
\author{E.~O.~Cohen} \affiliation{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978, Israel}
\author{S.~Covrig} \affiliation{Jefferson Lab, Newport News, VA}
\author{K.~Craycraft} \affiliation{University of Tennessee, Knoxville, TN}
%D                                                                                                                                                            
\author{B.~Dongwi} \affiliation{Hampton University , Hampton, VA}
\author{M.~Duer} \affiliation{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978, Israel}
\author{B.~Duran} \affiliation{Temple University, Philadelphia, PA}
\author{D.~Dutta} \affiliation{Mississippi State University, Miss. State, MS}
%E                                                                                                                                                            
%F                                                                                                                                                            
\author{E.~Fuchey} \affiliation{University of Connecticut, Storrs, CT}
%G                                                                                                                                                            
\author{C.~Gal} \affiliation{University of Virginia, Charlottesville, VA}
\author{T.~N.~Gautam} \affiliation{Hampton University , Hampton, VA}
\author{S.~Gilad} \affiliation{Massachusetts Institute of Technology, Cambridge, MA}
\author{K.~Gnanvo} \affiliation{University of Virginia, Charlottesville, VA}
\author{T.~Gogami} \affiliation{Tohoku University, Sendai, Japan}
\author{J. Golak} \affiliation{M. Smoluchowski Institute of Physics, Jagiellonian University, PL-30348 Krak\'ow, Poland}
\author{J.~Gomez} \affiliation{Jefferson Lab, Newport News, VA}
\author{C.~Gu} \affiliation{University of Virginia, Charlottesville, VA}
%H                                                                                                                                                            
\author{A.~Habarakada} \affiliation{Hampton University , Hampton, VA}
\author{T.~Hague} \affiliation{Kent State University, Kent, OH}
\author{O.~Hansen} \affiliation{Jefferson Lab, Newport News, VA}
\author{F. Hauenstein} \affiliation{Old Dominion University, Norfolk, VA}
\author{M.~Hattawy} \affiliation{Physics Division, Argonne National Laboratory, Lemont, IL}
\author{E.~Hughes} \affiliation{Columbia University, New York, NY}
\author{C.~Hyde} \affiliation{Old Dominion University, Norfolk, VA}
%I                                                                                                                                                            
\author{H.~Ibrahim} \affiliation{Cairo University, Cairo, Egypt}
%J                                                                                                                                                            
\author{S.~Jian} \affiliation{University of Virginia, Charlottesville, VA}
\author{S.~Joosten} \affiliation{Temple University, Philadelphia, PA}
%K                       
\author{H.  Kamada} \affiliation{Department of Physics, Faculty of Engineering, Kyushu Institute of Technology, Kitakyushu 804-8550, Japan}                                                                                                                
\author{A.~Karki} \affiliation{Mississippi State University, Miss. State, MS}
\author{B.~Karki} \affiliation{Ohio University, Athens, OH}
\author{A.~T.~Katramatou} \affiliation{Kent State University, Kent, OH}
\author{C.~Keppel} \affiliation{Jefferson Lab, Newport News, VA}
\author{M.~Khachatryan} \affiliation{Old Dominion University, Norfolk, VA}
\author{V.~Khachatryan} \affiliation{Stony Brook, State University of New York, NY}
\author{A.~Khanal} \affiliation{Florida International University, Miami, FL}
\author{D.~King} \affiliation{Syracuse University, Syracuse, NY}
\author{P.~King} \affiliation{Ohio University, Athens, OH}
\author{I.~Korover} \affiliation{Nuclear Research Center -Negev, Beer-Sheva, Israel}
\author{T.~Kutz} \affiliation{Stony Brook, State University of New York, NY}
%L                                                                                                                                                            
\author{N.~Lashley-Colthirst} \affiliation{Hampton University , Hampton, VA}
\author{G.~Laskaris} \affiliation{Massachusetts Institute of Technology, Cambridge, MA}
\author{W.~Li} \affiliation{University of Regina, Regina, SK , Canada}
\author{S. Li} \affiliation{University of New Hampshire, Durham, NH}
\author{H.~Liu} \affiliation{Columbia University ,New York, NY}
\author{N.~Liyanage} \affiliation{University of Virginia, Charlottesville, VA}
%\author{D.~Lonardoni} \affiliation{Facility for Rare Isotope Beams, Michigan State University, East Lansing, Michigan 48824, USA} \affiliation{Theoretical Di\
%vision, Los Alamos National Laboratory, Los Alamos, New Mexico 87545, USA}
%M                                                                                                                                                            
%\author{R.~Machleidt} \affiliation{Department of Physics,
%University of Idaho, Moscow, ID 83844, USA}
%\author{L.E.~Marcucci} \affiliation{Department of Physics ``E.\ Fermi'',
%University of Pisa, Italy} \affiliation{INFN, Pisa, Italy}
\author{P.~Markowitz} \affiliation{Florida International University, Miami, FL}
\author{R.~E.~McClellan} \affiliation{Jefferson Lab, Newport News, VA}
\author{D.~Meekins} \affiliation{Jefferson Lab, Newport News, VA}
\author{S.~Mey-Tal Beck} \affiliation{Massachusetts Institute of Technology, Cambridge, MA}
\author{Z-E.~Meziani} \affiliation{Physics Division, Argonne National Laboratory, Lemont, IL} \affiliation{Temple University, Philadelphia, PA}
\author{R.~Michaels} \affiliation{Jefferson Lab, Newport News, VA}
\author{M.~Mihovilovi\v{c}} \affiliation{University of Ljubljana, Ljubljana, Slovenia} \affiliation{Faculty of Mathematics and Physics, Jo\v{z}ef Stefan Institute, Ljubljana, Slovenia} \affiliation{Institut f\"{u}r Kernphysik, Johannes Gutenberg-Universit\"{a}t Mainz, DE-55128 Mainz, Germany}
%N                                                                                                                                                            
\author{V.~Nelyubin} \affiliation{University of Virginia, Charlottesville, VA}
\author{N.~Nuruzzaman} \affiliation{Hampton University , Hampton, VA}
\author{M.~Nycz} \affiliation{Kent State University, Kent, OH}
%O                                                                                                                                                            
\author{R.~Obrecht} \affiliation{University of Connecticut, Storrs, CT}
\author{M.~Olson} \affiliation{Saint Norbert College, De Pere, WI}
\author{L.~Ou} \affiliation{Massachusetts Institute of Technology, Cambridge, MA}
\author{V.~Owen} \affiliation{The College of William and Mary, Williamsburg, VA}
%P                                                                                                                                                            
\author{B.~Pandey} \affiliation{Hampton University , Hampton, VA}
\author{V.~Pandey} \affiliation{Department of Physics, University of Florida, Gainesville, FL}
\author{A.~Papadopoulou} \affiliation{Massachusetts Institute of Technology, Cambridge, MA}
\author{S.~Park} \affiliation{Stony Brook, State University of New York, NY}
\author{M.~Patsyuk} \affiliation{Massachusetts Institute of Technology, Cambridge, MA}
\author{S.~Paul} \affiliation{The College of William and Mary, Williamsburg, VA}
\author{G.~G.~Petratos} \affiliation{Kent State University, Kent, OH}
%\author{E. Piasetzky} \affiliation{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978, Israel}
\author{R.~Pomatsalyuk} \affiliation{Institute of Physics and Technology, Kharkov, Ukraine}
\author{S.~Premathilake}  \affiliation{University of Virginia, Charlottesville, VA}
\author{A.~J.~R.~Puckett} \affiliation{University of Connecticut, Storrs, CT}
\author{V.~Punjabi} \affiliation{Norfolk State University, Norfolk, VA}

%Q                                                                                                                                                            
%R                                                                                                                                                            
\author{R.~Ransome} \affiliation{Rutgers University, New Brunswick, NJ}
\author{M.~N.~H.~Rashad} \affiliation{Old Dominion University, Norfolk, VA}
\author{P.~E.~Reimer} \affiliation{Physics Division, Argonne National Laboratory, Lemont, IL}
\author{S.~Riordan} \affiliation{Physics Division, Argonne National Laboratory, Lemont, IL}
\author{J.~Roche} \affiliation{Ohio University, Athens, OH}
%S
\author{M.~Sargsian} \affiliation{Florida International University, Miami, FL}                                        
%\author{F.~Sammarruca} \affiliation{Department of Physics,
%University of Idaho, Moscow, ID 83844, USA}
\author{N.~Santiesteban} \affiliation{University of New Hampshire, Durham, NH}
\author{B.~Sawatzky} \affiliation{Jefferson Lab, Newport News, VA}
\author{E.~P.~Segarra} \affiliation{Massachusetts Institute of Technology, Cambridge, MA}
\author{B.~Schmookler} \affiliation{Massachusetts Institute of Technology, Cambridge, MA}
\author{A.~Shahinyan} \affiliation{Yerevan Physics Institute, Yerevan, Armenia}
\author{S.~\v{S}irca} \affiliation{University of Ljubljana, Ljubljana, Slovenia} \affiliation{Faculty of Mathematics and Physics, Jo\v{z}ef Stefan Institute,\
 Ljubljana, Slovenia}
\author{R.~Skibi\'nski}  \affiliation{M. Smoluchowski Institute of Physics, Jagiellonian University, PL-30348 Krak\'ow, Poland}
\author{N.~Sparveris} \affiliation{Temple University, Philadelphia, PA}
\author{T.~Su} \affiliation{Kent State University, Kent, OH}
\author{R.~Suleiman} \affiliation{Jefferson Lab, Newport News, VA}
\author{H.~Szumila-Vance} \affiliation{Jefferson Lab, Newport News, VA}
%T                                                                                                                                                            
\author{A.~S.~Tadepalli} \affiliation{Rutgers University, New Brunswick, NJ}
\author{L.~Tang} \affiliation{Jefferson Lab, Newport News, VA}
\author{W.~Tireman} \affiliation{Northern Michigan University, Marquette, MI}
\author{K. Topolnicki} \affiliation{M. Smoluchowski Institute of Physics, Jagiellonian University, PL-30348 Krak\'ow, Poland}
\author{F.~Tortorici} \affiliation{INFN Sezione di Catania, Italy}
%U                                                                                                                                                            
\author{G.~Urciuoli} \affiliation{INFN, Rome, Italy}
%V                                                                                                                                                            
%\author{M.~Viviani} \affiliation{INFN, Pisa, Italy}
%W                                                                                                                                                            
\author{L.B.~Weinstein} \affiliation{Old Dominion University, Norfolk, VA}
\author{H.  Wita{\l}a} \affiliation{M. Smoluchowski Institute of Physics, Jagiellonian University, PL-30348 Krak\'ow, Poland}
\author{B.~Wojtsekhowski} \affiliation{Jefferson Lab, Newport News, VA}
\author{S.~Wood} \affiliation{Jefferson Lab, Newport News, VA}
%X 
%Y                                                                                                                                                            
\author{Z.~H.~Ye} \affiliation{Physics Division, Argonne National Laboratory, Lemont, IL}
\author{Z.~Y.~Ye} \affiliation{University of Illinois-Chicago,
  Chicago, IL}
%Z                                                                                                                                                            
\author{J.~Zhang} \affiliation{Stony Brook, State University of New York, NY}


\collaboration{Jefferson Lab Hall A Tritium Collaboration}


